SF-UDA$^{3D}$: Source-Free Unsupervised Domain Adaptation for LiDAR-Based 3D Object Detection

3D object detectors based only on LiDAR point clouds hold the state-of-the-art on modern street-view benchmarks. However, LiDAR-based detectors poorly generalize across domains due to domain shift. In the case of LiDAR, in fact, domain shift is not only due to changes in the environment and in the object appearances, as for visual data from RGB cameras, but is also related to the geometry of the point clouds (e.g., point density variations). This paper proposes SF-UDA$^{3D}$, the first Source-Free Unsupervised Domain Adaptation (SF-UDA) framework to domain-adapt the state-of-the-art PointRCNN 3D detector to target domains for which we have no annotations (unsupervised), neither we hold images nor annotations of the source domain (source-free). SF-UDA$^{3D}$ is novel on both aspects. Our approach is based on pseudo-annotations, reversible scale-transformations and motion coherency. SF-UDA$^{3D}$ outperforms both previous domain adaptation techniques based on features alignment and state-of-the-art 3D object detection methods which additionally use few-shot target annotations or target annotation statistics. This is demonstrated by extensive experiments on two large-scale datasets, i.e., KITTI and nuScenes.

==> experiments_bk.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we report the results of our experimental evaluation in order to demonstrate the effectiveness of the proposed framework. % on the KITTI dataset from the source nuScenes dataset.
We first discuss the adopted datasets, the used evaluation metrics and the implementation details. Then, we report the results associated to our SF-UDA method, comparing with state of the art approaches. Finally, we shows the result of an ablation study to evaluate the impact on performance of our technical contributions.

%-------------------------------------------------------------------
\input{datasets}

\eli{questo sotto non si capisce}
As stated above, KITTI and nuScenes datasets consider different LiDAR ranges. Opposite to previous works \cite{wang2020train}, we do not force the ranges from  source and target domain to be the same, but instead, we only filter points based on the front camera, either in the CAM-FRONT space for nuScenes or in the rectified camera space for KITTI. To evaluate or to adapt the source model on the target dataset, we use the target ranges during the evaluation in order to detect or to fine-tune exploiting all the input information and to allow the adaptation to a new and unseen range. %Also the number of points deserves a particular attention since KITTI and nuScenes have an heavy difference in the mean number of points as reported in Tab. \ref{tab:sensors}. To tackle this difference, we follow the sampling strategy used in \cite{shi2019pointrcnn}

\textbf{Metrics.}
%\label{sec:metrics}
We used the official KITTI difficulties and metrics \cite{geiger2012we, geiger2013vision} for all the evaluations on the KITTI dataset. Detections are divided into Easy, Moderate and Hard based on the visibility of the object. For each evaluation, we report the Average Precision (AP) over the 3D Intersection over the union (IoU) with a IoU threshold of $0.7$ following the standard protocol of the KITTI benchmark \cite{geiger2012we, geiger2013vision}. Finally, we average over the three difficulty levels to provide an average (Avg) AP.

Similarly we consider the official nuScenes metrics \cite{nuscenes2019} for all the experiments on the nuScenes dataset. \eli{A wide range of metrics is proposed to investigate both the quality of the true positive detections and the ???}
In order to provide the same type of information of KITTI, in our experiments we considered the center-based definition of AP as used in the official nuScenes benchmark \cite{nuscenes2019} and reported both the AP at each of the four different distance thresholds of $[0.5, 1.0, 2.0, 4.0]$ meters and the final average (Avg) over the four thresholds.

\eli{Differently from other works \cite{wang2020train}... SE VOLGIAMO MOTIVARLO AGGIUNGERE ALTRA FRASE senò togliere}

% \subsubsection{Symmetric metric}
% Since the KITTI and nuScenes metrics report the same kind of information (AP) but over two different metrics (center-distance and 3D IoU), we adopt also a symmetric metric that allows to read the results on both the datasets form the same point of view. To this end, we adopt the well-known AP over the 3D IoU with thresholds at $[0.5, 0.7]$. Moreover, we report also the average (Avg-3D) over the two thresholds.

%\subsection{Experimental setup}
%\label{sec:setup}


\begin{table*}[ht]
    \centering
    %% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
    \begin{tabular}{ccccccccccc}
      \toprule
        \textbf{Method} & \textbf{Information} & \textbf{Fine-tuning} & \textbf{Easy} & \textbf{Moderate} & \textbf{Hard} & \textbf{Avg-AP}\\ \midrule 
        Source & Supervised & \xmark & 0.273 & 0.196 & 0.188 & 0.219\\ \midrule
        OT \cite{wang2020train}& Weakly & \xmark & 0.199 & 0.166 & 0.153 & 0.173\\
        FS \cite{wang2020train} & Supervised & \xmark & 0.506 & 0.436 & 0.396 & 0.446\\
        ES-GT= ES with GT scale  & Weakly & \xmark & 0.549 & 0.386 & 0.370 & 0.435\\ 
        GTS=ES+finetuning & Weakly & \cmark &  0.626 & 0.456 & 0.414 & 0.499\\
        \midrule
        AdaBN \cite{li2016revisiting} & Unsupervised & \xmark & 0.277 & 0.200 & 0.188 & 0.222\\ 
        No scale + FT & Unsupervised & \cmark & 0.396 & 0.275 & 0.236 & 0.306\\
        No scoring + FT & Unsupervised & \cmark & 0.289 & 0.200 & 0.180 & 0.223\\
        ES=ES with estimated scale & Unsupervised & \xmark & 0.465 & 0.347 & 0.299 & 0.370\\ 
        % EOS-2=OS with estimated scale & Unsupervised & \xmark & 0.503 & 0.366 & 0.314 & 0.394\\ 
        % EOS-3=OS with estimated scale& Unsupervised & \xmark & 0.462 & 0.343 & 0.301 & 0.369\\ 
        \midrule
        Ours top-1 & Unsupervised & \cmark & 0.589 & 0.414 & 0.388 & 0.464\\ 
        Ours top-3 & Unsupervised & \cmark & \textbf{0.688} & \textbf{0.498} & \textbf{0.450} & \textbf{0.545}\\ 
        Ours top-5 & Unsupervised & \cmark & 0.657 & 0.479 & 0.427 & 0.521\\ 
        \midrule
        Target & Supervised & \xmark & 0.873 & 0.769 & 0.760 & 0.801\\ 
        \bottomrule
    \end{tabular}
    \caption{Adaptation results on nuScenes$\rightarrow$KITTI.\\
    \fg{
    A few concerns:\\
    - 3rd and 4th entry need a reference to \cite{wang2020train}, and also ES=OS with estimated\\
    - in the second box I would include adabn (already) as well as ours top-x\\
    - place all other entries in the third box (apart from target, in its own), here basically ablation studies, this should be similar to table kitti to nuscenes.
    }
    }
    \label{tab:nusc2kitti}
\end{table*}

\textbf{Implementation details.}
%\label{sec:implementation}
We implemented our franework in PyTorch and used the publicly available PointRCNN implementation as 3D detector \eli{missing footnote}. For training and evaluating our method, we run all our experiments on a DGX-1 server (8 Nvidia Tesla V-100 GPUs) and on a Lambda Blade server (8 NVidia Quadro RTX 6000 GPUs). 
The source training have been performed with the ADAM  optimizaiton algorithm and one-cycle policy for 200 and 70 epochs for the RPN and RCNN respectively, with a batch size of 64 and 32 respectively, and with a maximum learning rate of $0.02$ as in \cite{shi2019pointrcnn}. Similarly, during the target fine-tuning we kept the same training setup with the only difference that we train the RPN for 100 epochs with a maximum learning rate of $0.002$.
During the scale search, we use a grid size parameter $\epsilon=0.3$ and we employ a stride $s=0.075$ along each axis. We thus obtain a solution space of dimension of $L=125$.
As for the tracking by detection module, we use the publicly available code in \cite{weng2019baseline} and change the tracker hyper-parameters qualitatively to adapt to PointRCNN and to the noisy detections obtained with the source model on target data. To this aim, we set on both the datasets the initialization threshold to $2$ matched detections and the death threshold to $2$ missed detections. Finally, regarding the pseudo-annotation procedure, we annotate four times the target dataset for each confidence threshold in the list $[0.05, 0.1, 0.2, 0.3]$ and use an NMS IoU threshold of $0.1$ to merge pseudo-annotations.


\textbf{Baseline methods.}
%\label{sec:exp-methods}

\fg{This section may need to separate methods from ablation studies..}
\cris{Agree, we need to decide what goes in Ablations}
Although we are the first in proposing an UDA and source-free method for 3D detection, for a fair comparison we report also the results obtained by applying other existing weakly-supervised and UDA methods implemented and adapted to our source-free setup or adapted to the scenario of 3D detection.
\fg{change the tone: we are the first on the source-free UDA.. we get baselines from other applicable techniques.. however we should distinguish what we bring to Lidar (adabn) and what we find there already \cite{wang2020train}.}

\noindent\textit{AdaBN}\cite{li2016revisiting}: this method is meant for UDA in classification but we adapted it to the detection task by updating the batch-normalization (BN) parameters before testing the source model on the target validation set. To this end, we forward the target training set in the source model to update the BN parameters of PointRCNN and finally evaluate over the target validation set.

\noindent\textit{Output Transformation (OT)}\cite{wang2020train}: the method consists in exploiting the weakly supervised information of the average dimensions of objects in the source and target domain to transform the predictions of source model on the target data. Although this method is not fairly unsupervised, we report it being the closest to our setup. Following \cite{wang2020train}, we added to each target prediction of the source model the difference between the average sizes of objects of the two domains.

\noindent\textit{Few-Shot fine-tuning (FS)}\cite{wang2020train}: the method foresees the fine-tuning on a set of 10 randomly sampled annotated target data. Following \cite{wang2020train}, we run 5 times the FS fine-tuning over differently sampled samples and report the average performance.

\noindent\textit{Estimated Scaling (ES)}: exploiting the predicted top-1 $\omega^*$ as described in Sec. \ref{sec:method}, we evaluate the target performance by applying the best scaling triplet to scale the input and re-scale the predictions at test-time only.
\fg{this is basically the same as \cite{wang2020train} but with estimated scale? then should say so..}
\cris{no it's different, in \cite{wang2020train} they do not touch the input, here we apply our scale and detect procedure but at test time only}

\fg{methods below this point are actually ablation studies? we should distinguish. we'd claim as ours and ablation studies those which use our pipeline, I imagine.}
\cris{yes, if we want to puyt them in ablation yes}

\noindent\textit{Ground Truth Scaling (GTS)}: we take advantage of the weak supervision in knowing source and target statistics and perform the auto-annotation pipeline by substituting the randomly sampled $\omega_{tmp}$ with the ratios used in OS. After the annotation, we perform a fine-tuning over the auto-annotated target dataset.

\noindent\textit{No scale}: we apply our pipeline without any scaling procedure and by using source model detections as pseudo-annotations. We include this variant so as to show the importance of scaling during pseudo-annotation.

\noindent\textit{No scoring}: we apply our pipeline without any scoring procedure for the scaling parameters and by using the scaling transformation as random augmentations during the pseudo-annotation phase.


\subsection{Adaptation results}
\label{sec:exp-adaptation}
\cris{we need to decide what to put in ablations}
For a fair comparison of the performance with existing methods, we run the experiments from nuScenes to KITTI by using the same split of \cite{shi2019pointrcnn}. In Tab. \ref{tab:nusc2kitti}, we report the results obtained in the nuScenes$\rightarrow$KITTI task for the KITTI class \textit{Car} with our method in the top-1, top-3 and top-5 configuration. Here, we compare our performance also with the weakly-supervised methods \textit{FS} and \textit{OT}\cite{wang2020train} showing that our pipeline is capable to reach better performance than the compared weakly and few-shot supervised methods by a large margin.
Another interesting outcome is the $0.080$ average AP improvement obtained by using top-3 and top-5 intervals compared with the top-1 and \colorbox{red}{GTS} versions. The contribution of this result is twofold. First, the better numbers of top-3 show that the relaxation is useful in order to move around the optimal scaling values that could not work for certain frames. Second, the better numbers of both top-3 and top-5 show that the supervised information of target and source average dimensions used in GTS might not include the information coming from the surround of the objects.
Interestingly, also at test time the scaling parameters produce an improvement in the metrics and this further proves how the scale and detect step is useful for both obtaining new detections and better detections compared to the source model. We further investigated this comparison in Sec. \ref{sec:abl-pseudo}.
For a qualitative evaluation of this improvement, we report in Fig. \ref{fig:detections} the comparison between the detections with $\Phi_\mathcal{S}$ and with the final $\Phi_\mathcal{T}$. As visible, the improvement after adaptation is sensible both in terms of better retrieved boxes and more detected objects. Please refer to the Supplementary Material for more qualitative examples.
Finally, it is worth noting how important is the fine-tuning procedure for obtaining a better adaptation. This further proves the effectiveness of the scaling procedure in obtaining better and more informative pseudo-annotations.

\begin{figure*}
    \centering
    \includegraphics[scale=0.4]{images/detections/detections.pdf}
    \caption{\textbf{Before (upon) and after (below) adaptation.} After adaptation, performance improves and more objects are detected.}
    \label{fig:detections}
\end{figure*}


